DANLI: Deliberative Agent for Following Natural Language Instructions

Recent years have seen an increasing amount of work on embodied AI agents that can perform tasks by following human language instructions. However, most of these agents are reactive, meaning that they simply learn and imitate behaviors encountered in the training data. These reactive agents are insufficient for long-horizon complex tasks. To address this limitation, we propose a neuro-symbolic deliberative agent that, while following language instructions, proactively applies reasoning and planning based on its neural and symbolic representations acquired from past experience (e.g., natural language and egocentric vision). We show that our deliberative agent achieves greater than 70% improvement over reactive baselines on the challenging TEACh benchmark. Moreover, the underlying reasoning and planning processes, together with our modular framework, offer impressive transparency and explainability to the behaviors of the agent. This enables an in-depth understanding of the agent's capabilities, which shed light on challenges and opportunities for future embodied agents for instruction following. The code is available at https://github.com/sled-group/DANLI.

==> sections/longer-2-related_work.tex <==

% \paragraph{Natural Language Instruction Following} % - Shane, Emily, Martin} 

Past approaches for embodied instruction following have used
% recurrent networks and transformers
neural networks to predict sequences of actions directly from language instructions, with efforts toward 
% navigation fidelity \cite{jain-etal-2019-stay}, 
progress monitoring \cite{ma2019selfmonitoring,ma2019theregretful,Zhu_2020_CVPR}, grounding to visual surroundings \cite{jain-etal-2019-stay,hu-etal-2019-looking,tan-etal-2019-learning,storks-gao-thattai-tur-2021-embodied}, and targeted data augmentation \cite{friedSpeakerFollowerModelsVisionandLanguage2018,majumdar2020improving,Suglia2021EmbodiedBA,pashevich2021episodic}.
% Later work harnessed transformers to enable multimodal, disembodied pre-training at scale \cite{majumdar2020improving,suglia2021embodied}, augmentation of instructions \cite{pashevich2021episodic}, 
The topics most relevant to this work include: \textit{semantic scene representation}, \textit{hierarchical policies}, and \textit{symbolic planning}.



% To combine and improve upon more recent advances, we propose a \textit{hierarchical}, neuro-symbolic deliberative agent which utilizes a novel \textit{symbolic planning} algorithm over richer \textit{scene representations} to execute tasks.




% Talk about previous work that models a reactive agent (e.g. those previous work on ALFRED: HiTUT, HLSM \cite{blukis2022hlsm}, E.T. \cite{pashevich2021episodic}, etc) on ALFRED etc. We instead modeling a planning-based agent. Talk about other planning-based solution and how we differ from them (e.g. \cite{zhou2021hierarchical}). Talk about how the EDH setting in TEACh differs from instruction following (e.g. need to infer the task progress / have to understand a mixture of high-level and low-level instructions etc). 

% Draft so far
% Recent years have seen the creation of various benchmark datasets for embodied instruction following requiring navigation in spatial environments and manipulation of objects~\cite{mattersim,thomason:arxiv19,reverie,shridhar2020alfred,padmakumar2021teach}.
% and other household tasks requiring manipulation of objects~\cite{shridhar2020alfred,padmakumar2021teach}. 

% Later approaches introduce hierarchical task learning~\cite{zhang2021hitut}, planning-based agents \cite{zhou2021hierarchical}, and persistent semantic spatial representations~\cite{blukis2022hlsm} to the problem for more data-efficient and generalized training.
% To combine and improve upon these past advances, we propose a neuro-symbolic deliberative agent which utilizes a novel symbolic planning algorithm over richer scene representations to execute tasks.
% This is especially helpful for interpreting dialog history (used as instructions in our task), which requires us to interpret both high-level and low-level instructions that may occur, and reconcile them with task progress.



% Then various flavors of seq2seq models - have some review from an older paper that will cover some of it
% \citet{friedSpeakerFollowerModelsVisionandLanguage2018} speaker follower
% Auxiliary tasks/objectives:1
% navigation fidelity \citet{jain-etal-2019-stay} 
% progress monitor \citet{ma2019selfmonitoring} 
% Backtracking \citet{ma2019theregretful} 
% Object detection \citet{hu-etal-2019-looking}
% Many auxiliary tasks \citet{Zhu_2020_CVPR}
% Goal localization? (Storks et al. 2021)
% Newer transformer based models HiTUT, HLSM \cite{blukis2022hlsm}, E.T. \cite{pashevich2021episodic}, VLNBERT? EmBERT? \citet{majumdarImprovingVisionandLanguageNavigation2020}




\paragraph{Semantic Scene Representation} A strong world representation is necessary for spatial and task-structure reasoning in embodied AI. While prior work \cite{pashevich2021episodic,Nguyen2021LookWA,Suglia2021EmbodiedBA,Khandelwal2021SimpleBE} converts visual observations of the environment to vector representations and uses them directly for action prediction, these purely numerical representations are not interpretable, posing difficulties for 
symbolic planning.
% (such as a PDDL planner) 
% which operates on a symbolic domain. 
Some methods have instead applied rich spatial representations to the problem. 3D scene graphs~\cite{3dsg2019, 3dsg2020, pmlr-v164-li22e, pmlr-v164-agia22a} are one example, but they abstract away important details about object position and size needed for low-level motion planning.
Other works build a semantic map of the environment with occupancy and object class information \cite{chaplot2020object, saha2021modular, blukis2022hlsm, min2021film},
% for better performance on embodied instruction following tasks. These methods accumulate information gathered from visual observations of the environment by building a % 2D or 3D 
% semantic map containing occupancy and object class information, 
then use it to inform downstream reasoning tasks.
% These methods differ from the pure vectorized representations in that they accumulate the information gathered from visual observations of the environment by building a 2D/3D semantic map. The map contains both occupancy and semantic information, meaning we know which cells in the map are occupied and which classes of objects are occupying them. The semantic map is then input into subsequent modules in the system for spatial and logical reasoning. The intermediate map gives a more interpretable representation for human. Our method is based on this family of semantic map representation but differs from existing work in that 
We follow the latter approach, but unlike prior work, our semantic map additionally models object \textit{instance} and \textit{physical state}
% , incorporating these labels into the resulting map 
to inform planning where a task involves multiple instances of an object class or physical state changes. Further, we supplement our visually-informed semantic map with spatial information extracted from dialog utterances.




\paragraph{Hierarchical Policies} 
%Refer to the related work in \cite{sharma2021skill, zhang2021hitut}. 

Hierarchical policy learning and temporal abstraction have long been studied in reinforcement learning \cite{ hier_old2, hier_old3,hier_old4,hier_old5,hier_old6,hier_old7,hier_old8} to uncover the inherent structures of complex tasks. More recently, they have brought improvements in natural language instruction following over direct sequence-to-sequence approaches \cite{sharma2021skill, zhang2021hitut, zhou2021hierarchical, blukis2022hlsm} by predicting actions in two stages: 1) subgoal prediction from instructions, and 2) action execution given subgoals.
While prior work applies planning at the high level for subgoal prediction, a reactive approach is still used for low-level action execution. As such, we build a deeply deliberative agent by using specialized planners for interaction and navigation actions based on our spatial-symbolic world representation, thus enabling more reliable subgoal completion. 
% Here, we split action execution into two separate branches for interaction and navigation, each with specialized planners. 
For subgoal prediction, we instead propose a powerful sequence-to-sequence task monitor informed by the dialog and action history to track completed and upcoming subgoals, and interface with these planners.
% \jycc{a bit confusing. for manipulation and navigation separately? }
% each using separate prediction and planning modules with specialized inductive bias. 
% Further, while prior work has generated plans for tasks based only on subgoals (the highest level of hierarchy), we apply planning at the low level to predict actions within these two branches for more reliable subgoal completion. Meanwhile, we use a powerful sequence-to-sequence task monitor informed by the dialog and action history to track completed and upcoming subgoals and interface with these planners.
% introduce three levels of hierarchy: subgoal prediction, interaction planning, and navigation planning, and use different prediction and planning modules with proper inductive bias to achieve advanced performance. 
% This setup 
% %of our approach 
% offers more insight into our system's planning, operation, and navigation capabilities than past work.


% considers complex contextual interactions between symbols.

% introduce two other levels of hierarchy in the PDDL-based \cite{McDermott1998PDDLthePD} planner, \textit{i.e.}, interaction planning and navigation planning.

% Compared to classical planning work: we focus on complex embodied 3D domain with partial observability. Need to compared to \cite{lamanna2021online}: (1) they only have navigation + open/close while we have more complex physical state change and task goals. (2) we learn the task goal from natural language. (3) we have some novelty in the design of planning algorithm (e.g. incorporate searching for a specific object into the planning loop) 
% Most task planning work does not operate end-to-end in embodied 3D domains, and thus lose 
% \cite{galindo2004improv, kavraki1996prm, galindo2008semmap}.
% Unlike their work, ours handles complex 3D environments with partial observability.
% OGAMUS \cite{lamanna2021online} 
% PIGLeT \cite{zellers2021piglet} 
% related work to cite:
% blanket cite classical task planning work
    % take from related work of prior papers
% lamanna et al
% taskography?
% piglet?
% key assets and features of our symbolic planner:
% interpretable
% capture complex physical state changes (including contextual interactions) and task goals
% learned subgoals from natural language
% plans for all single subgoals
% planning loop design decisions: object search... is this worth mentioning?




% (1) we add object \emph{instance} labels beyond semantic labels; (2) we additionally model \emph{physical state} for each object instance. 

% While 3D scene graphs are another strong representation \cite{3dsg2019, 3dsg2020, pmlr-v164-li22e, pmlr-v164-agia22a}, they abstract away fine-grained details such as object position and size, which are important for low-level motion planning.

% While another family of representation is 3D scene graph \citep{3dsg2019, 3dsg2020, pmlr-v164-li22e, pmlr-v164-agia22a}. These methods represent objects and their 3D spatial relations with nodes and edges in a graph. Graph representation provides a good abstraction and might facilitate task-structure reasoning but poses challenges for spatial reasoning since it hides away finer-grain details such as object centroids and sizes, which are important for manipulation actions.   

% \todo{Jed: Write section.} One directions: semantic map HLSM, FILM, Chaplot, related work from HLSM paper. Our approach differs in: (1) we have object instance labels beyond semantic labels; (2) we additionally model physical state for them. The other direction: 3DSG: in our representation we have additional spatial information and also state changes to reflect environment dynamic. 


\paragraph{Symbolic Planning}
Symbolic planning has been extensively studied in the classical AI literature and applied in robotics, where  
% \nikhil{@Joyce do you mind elaborating on what the goal of this first sentence is? The next sentence roughly describes what symbolic planning tries to do, but it seems like this first sentence also wants to do that?}
% \jycc{@nikhil..ah, just want to acknowledge that we know this is a classical AI topic. need to rephrase the first sentence a little bitl}
% Work in robotic task completion often involves symbolic planning, in which 
environment entities, actions, and goals are represented as discrete symbols \cite{McDermott1998PDDLthePD,galindo2004improv, kavraki1996prm, galindo2008semmap}.
Recent work aims to learn these symbols from language \cite{zellers2021piglet, silver2021learn, MacGlashan2015GroundingEC} and vision \cite{lamanna2021online,xu2022sgl}.
Unlike these efforts, our approach combines both modalities by learning symbolic task goals from natural language, and leveraging a persistent scene representation based on detected object instances. 
% As such, our algorithm can capture more complex, contextual interactions between entities dependent on their physical states.
Further, unlike past work, we optimize our approach for embodied instruction following by adding capabilities to search for missing objects, knowledgeably prune the search space, and recover from failed actions.
% enabling a goal-oriented search function for missing objects, and 

% We note that similar neuro-symbolic planners, such as OGAMUS \cite{lamanna2021online}, are unable to perform such goal-oriented searches online.
% This mitigates errors from learning the planning domain directly from language or vision.
% , e.g. if a plate is moved underneath a toggled faucet, then the planner should assume its state is changed to \texttt{isClean}.
% Our approach deviates from classical task planning because it leverages symbols learned from language and operates in a complex, embodied 3D environment with partial observability. 
% Recent work looks to learn these symbols, either in the problem's domain \cite{zellers2021piglet, silver2021learn} or its goals \cite{MacGlashan2015GroundingEC}. 
% Particularly similar to ours is OGAMUS \cite{lamanna2021online}, which also operates on top of the iTHOR simulator \cite{kolve2017ai2thor}. The main contribution of this work was a framework to construct a symbolic planning domain (as in PDDL) online and use it to solve ObjectGoal \cite{anderson2018eval} tasks. Our approach differs from OGAMUS in that we encode 
% more complex physical states and task goals, such as toggling, slicing, and pouring, as opposed to only navigation, opening/closing, and stacking objects. We also learn our task goals from natural language and leverage a learned scene representation for objects, as opposed to simply learning the planning domain itself from perception, which allows error when learning even simple transitions between symbols.

%Further, as we have introduced two levels of hierarchy to the traditional PDDL-based planner~\cite{McDermott1998PDDLthePD}, our approach necessitates more complex, contextual interactions between symbols.

